Raccoon: Multi-stage Diffusion Training with Coarse-to-Fine Curating Videos

Text-to-video generation has demonstrated promising progress with the advent of diffusion models, yet existing approaches are limited by dataset quality and computational resources. To address these limitations, this paper presents a comprehensive approach that advances both data curation and model design. We introduce CFC-VIDS-1M, a high-quality video dataset constructed through a systematic coarse-to-fine curation pipeline. The pipeline first evaluates video quality across multiple dimensions, followed by a fine-grained stage that leverages vision-language models to enhance text-video alignment and semantic richness. Building upon the curated dataset's emphasis on visual quality and temporal coherence, we develop RACCOON, a transformer-based architecture with decoupled spatial-temporal attention mechanisms. The model is trained through a progressive four-stage strategy designed to efficiently handle the complexities of video generation. Extensive experiments demonstrate that our integrated approach of high-quality data curation and efficient training strategy generates visually appealing and temporally coherent videos while maintaining computational efficiency. We will release our dataset, code, and models.

==> sec/3_method.tex <==
\section{Method}
\label{sec:method}


\subsection{Dataset}

The existing datasets for video generation training currently suffer from three main issues that significantly impact the quality and utility of the generated content:

\mypara{Low Quality of Video }
1.Temporal Inconsistency: Errors in scene transition detection algorithms lead to low temporal consistency within the video content, disrupting the logical sequence of events.
2.Static Videos: Some videos exhibit minimal to no movement, resulting in static scenes that do not effectively convey dynamic or evolving narratives.

\mypara{Low Quality of Caption }
1.Caption Generation Errors: The instability of the video MLLM model often results in the generation of inaccurate captions. Common issues include frame-by-frame descriptions, incorrect generation of EOS tokens, and captions that completely misdescribe the video content.
2.Lack of Detailed Descriptions: Compared to the Panda70M dataset, which averages 13 words per video caption, our dataset aims for more detailed captions with an average word length of 89. This discrepancy highlights the need for more granular and descriptive captions in our training data.
3.Low Video-Text Alignment: There is often a significant misalignment between the semantic and temporal descriptions in the captions and the actual video content. This inconsistency undermines the effectiveness of the captions in accurately representing the video narratives.

\subsubsection{Data Collection}

For our model training, we adopted a joint training approach utilizing both images and videos. In this context, we compiled a dataset consisting of 40 million images and 8 million videos. Moreover, to foster further research and development in the field, we have made 1 million videos from this dataset openly available to the public.
%Image Data 
Our image dataset was meticulously curated from multiple sources. We utilized images from the laion5B, JourneyDB and COYO datasets, supplemented by additional data collected and cleansed from various internet sources. Through these efforts, we have successfully compiled a high-quality training dataset comprising 40 million images, specifically designed to enhance text-to-image generation models.
%Video Data  -> VidGen
For the video component, we leveraged the HD-VILA dataset to construct the VidGen dataset. This process involved the utilization of 3.8 million high-resolution, long-duration videos from HD-VILA, which were then segmented into 108 million video clips. These clips were carefully tagged and sampled for further use. The VILA model was subsequently employed for video captioning tasks. To ensure the accuracy and relevance of the captions, we applied a Large Language Model (LLM) to refine and curate the captions, addressing any discrepancies identified in the initial data curation phase.



\subsubsection{Video Coarse Curation}
To achieve efficient data curation with limited computational resources, we propose multi-stage data curation pipeline, which involves scene splitting, video tagging, filtering and sampling to reduce the computational cost in subsequent stages. 

\mypara{Scene Splitting}
Motion inconsistencies, such as scene changes and fades, are frequently observed in raw videos.
However, since motion inconsistencies directly cut off the video semantics, text-to-video models are significantly sensitive to and confused by them, leading to heavy impairment on training efficiency.
To alleviate their impairment, we follow the prior research~\citep{blattmann2023svd, chen2024panda,opensora} to utilize PySceneDetect~\citep{pyscenedetect} in a cascading manner to detect and remove scene transitions in our raw videos. 

\mypara{Video Tagging}
In order to construct a dataset suitable for training text-to-video models, the data must meet the following criteria: high-quality videos, balanced categories, and strong temporal consistency within the videos. To achieve this goal, we first need to tag each splitted video clip. Subsequently, these tags serve as the basis for curating and sampling.

\textbf{Video Quality.}
The visual quality of videos is of paramount importance for the efficient training of text-to-video models. 
In order to enhance the quality of generated videos in text-to-video generation, we adopt a strategy of filtering out videos with low aesthetic appeal and high OCR scores. 
In this context, we employ the LAION Aesthetics model to predict and evaluate aesthetic scores, thereby ensuring a superior quality of training data.
Particularly, the aesthetics models can also filter out visually abnormal videos, such as videos with irregular color distribution or weird visual elements.

\textbf{Temporal Consistency.} 
Incorrect scene splitting in videos can significantly impair the effectiveness of model training. High temporal consistency is a crucial characteristic required for the training data in text-to-video models. To ensure this, we utilize the CLIP model to extract visual features and assess temporal consistency. This assessment is achieved by calculating the cosine similarity between the starting and ending frames of video clips, thereby providing a quantitative measure of continuity and coherence.

\textbf{Category} 
The HD-VILA-100M video dataset displays significant imbalances across its categories, resulting in less than optimal performance of video generation models for these categories. To tackle this issue, we deploy predefined category tags to label each video, with the assistance of the CLIP model. Specifically, we extract the CLIP image features from the initial, middle, and final frames of each video, compute their average, and then determine the similarity between these averaged image features and the textual features associated with each tag. This methodology enables us to assign the most fitting tags to each video.

\textbf{Motion.} 
We employ the RAFT~\citep{teed2020raft} model to predict the optical flow score of videos. As both static videos and those with excessively fast motion are detrimental for training text-to-video models, we filter out these videos based on their optical flow scores.

\mypara{Sampling}

\begin{figure}[ht]
    \centering
    \includegraphics[width=\columnwidth]{sec/figs/data_distribution.pdf}
    \caption{Distribution of curated data.}
    \label{fig:data_distribution}
\end{figure}

By employing tags associated with visual quality, temporal consistency, category, and motion, we undertook the task of filtering and sampling. The curated data distribution across multiple dimensions in our dataset is depicted in Figure \ref{fig:data_distribution}. This figure clearly indicates that videos characterized by low quality, static scene, excessive motion speed, and those demonstrating inadequate alignment between text and video along with poor temporal consistency were systematically removed. Concurrently, we have ensured a relatively even distribution of samples across diverse categories.

\subsubsection{Video Fine Curation}
Building upon the video data curated during the coarse curation phase, we first employed the Video MLLM model to generate high-quality captions for each video. Subsequently, these captions were subjected to further refinement using a Large Language Model (LLM). This additional filtering step was crucial for removing any captions that were unsuccessfully generated or deemed unsuitable for video generation training.

\mypara{Data Captioning}

The quality of video captions exerts a critical influence on text-to-video model, while the captions in the HD-VILA-100M dataset demonstrate several problems, including misalignment between text and video, inadequate descriptions, and limited vocabulary use. To enhance the information density of the captions, we employ the cutting-edge vision-language model, VILA~\citep{lin2024vila}. 
Owing to the remarkable video captioning ability of VILA, we have significantly enhanced caption quality. 
After captioning, we apply clip score to filter out the text-video pairs with low similarity.

% caption result 
We present a vocabulary analysis in Table \ref{tab:dataset_summary}, where we identify valid distinct nouns and valid distinct verbs as those that appear more than 10 times in the dataset. Utilizing the VILA model on the HD-VILA-100M dataset, we have generated the enhanced HD-VILA-100M dataset. In the Panda-70M dataset, there are 270K distinct nouns and 76K distinct verbs; however, only 16.1\% and 19.2\% of these meet the validity criteria, respectively. 
Captions generated using VILA substantially enhance the valid ratio as well as the average count of nouns and verbs per video, thereby increasing the conceptual density.

\begin{table}[ht]
\centering
\begin{tabular}{l|cccc}
\toprule
\textbf{Dataset}      & \textbf{VN/DN}    & \textbf{VV/DV}    & \textbf{Avg N} & \textbf{Avg V} \\
\midrule
Pandas-70M            & 16.1\%            & 19.2\%            &   4.3             &   1.9      \\
\textbf{Ours}                  & 20.3\%            & 41.1\%            &   22.5             &   15.9     \\
\bottomrule
\end{tabular}
\caption{Statistics of noun and verb concepts for different datasets. 
VN: valid distinct nouns (appearing more than 10 times); DN: total distinct nouns; Avg N: average noun count per video.
VV: valid distinct verbs (appearing more than 10 times); DV: total distinct verbs; Avg N: average verbs count per video.}
\label{tab:dataset_summary}
\end{table}

\mypara{Video-Text pair Curation }
During the coarse curation stage, predictive scoring utilizes the CLIP score to filter out certain impurities, such as temporally inconsistent videos. However, this method is not infallible and fails to address several prevalent issues that commonly undermine video captions:
Scene Splitting Error: The model struggles with scene transitions, often failing to recognize when one scene ends and another begins.
Failed EOS Token Generation: Occasionally, the model does not correctly conclude the captioning process, which results in the generation of looping or repetitive tokens.
Frame-level Description: The model often fails to understand the dynamic relationships between frames, leading to isolated descriptions for each frame. As a result, the generated captions lack coherence and do not accurately represent the video's overall narrative and action sequence.
To address these data curation challenges, manual annotation represents a potential, albeit cost-prohibitive, solution. Fortunately, recent advancements in large language models (LLMs) offer a promising alternative. By employing an LLM, errors in captions produced by Multi-Modal Language Models (MLLMs) can be accurately identified, including issues related to scene transitions, repetitive content, and frame-level descriptions. Models such as LLAMA3 have demonstrated exceptional proficiency in these tasks, providing a viable alternative to manual annotation.
In our efforts to isolate and eliminate discrepancies in video-text alignment and temporal consistency, we utilized the advanced Language Model, LLAMA3.1. This model conducted a meticulous analysis of the captions, leading to significant improvements in the quality of the text-video pairs. The effectiveness of this fine curation process is clearly demonstrated in Figure \ref{fig:caption_compare}. Our study primarily focuses on three critical issues: Scene Transition (ST), Frame-level Generation (FLG), and Reduplication (Redup).

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{sec/figs/caption_compare.pdf}
    \caption{Caption Curation Result. Employing Llama3.1 to curate video captions, as produced by VILA, results in a significant improvement in the quality of the training dataset. This is specifically evidenced through improvements in video temporal consistency and alignment between text and video. Consequently, this method facilitates notable improvements in the performance of the text-to-video model.}
    \label{fig:caption_compare}
\end{figure}


\subsection{Training Strategy}

\ourmethod is trained with four stages, namely semantic learning, temporal learning stage, Multi Resolution \& Duration Training, and high-aesthetic finetuning. The overall pipeline is presented in Fig. X. We describe details as follows.

\mypara{Stage 1: Semantic Learning} Leveraging a pre-trained text-to-image model significantly accelerates the convergence speed of text-to-video training and enhances semantic understanding capabilities. By initially training on large-scale image-text pair datasets, we effectively enrich the semantic modules essential for video generation. This pre-training with a vast corpus of image data allows the model to assimilate a broader spectrum of semantic information, thereby improving the video model's ability to interpret and generate content with greater semantic depth. Consequently, the video generation model can focus more on mastering temporal dynamics while relying on robust foundational knowledge, leading to more efficient and nuanced training outcomes. 
Utilizing a pre-trained Causal 3D VAE, we can establish a shared and unified latent representation for both images and videos. This compressed visual representation is critical for generative modeling across both mediums. The unified approach is particularly advantageous due to the scarcity of labeled video data, which makes image pre-training and joint image-video learning preferable. In our model, images are treated as single frames of video, allowing the semantic module parameters from image pre-training to be fully applicable to subsequent video generation tasks. Therefore, during this training phase, we focus solely on training the semantic module parameters within the video generation model through the text-to-image tasks.

\mypara{Stage 2: Temporal Learning} 
% low resolution & short duration videos 
Having completed the training of the semantic components within our generative model during Stage 1, we now progress to the learning of the temporal modules by jointly training with images and videos. This phase is crucial for mastering the dynamics essential for video generation. To reduce the training costs associated with the temporal modules, we employ low-resolution images and short-duration videos for joint training. For this purpose, we utilize our internally cleansed dataset comprising 256x256 40 million image-text pairs and 256x256 under 2s 8 million video-text pairs.
This strategy enables the temporal module to converge rapidly, enhancing the generative model's capability to produce videos with strong textual and temporal consistency. By optimizing the resolution and duration of the training media, we maintain computational efficiency while ensuring that the model learns to accurately interpret and generate time-sensitive visual narratives. This approach not only streamlines the training process but also improves the quality and coherence of the generated video content.


\mypara{Stage 3: High Resolution and Long Duration Training}
Following the completion of training in Stage 2, the model is capable of generating low-resolution and short-duration videos. However, these outputs are still insufficient to meet current demands for higher quality media. Consequently, we have shifted our focus towards training the model using high-resolution images and high-resolution, long-duration videos. This strategy is designed to enhance the model's capability to produce videos that are both high in resolution and extended in duration.
By employing high-quality visual data in the training process, we aim to significantly improve the model's performance and output quality. This approach not only addresses the limitations observed in earlier stages but also aligns with the growing expectations for richer and more detailed video content in various applications, from entertainment to educational fields. The transition to higher resolution and longer video formats is crucial for achieving a more realistic and engaging viewer experience, making this phase of training a pivotal step in the development of our generative model.

\mypara{Stage 4: High-quality Fine-tuning}
During Stage 3 of our training, the generative model is capable of producing high-resolution, long-duration videos. However, the quality of these videos tends to be relatively random and unstable. To address this challenge and guide the model towards generating videos that not only meet technical specifications but also exhibit high visual aesthetics, we implement an additional finetuning step using the diffusion model.
For this finetuning process, we utilize a carefully curated set of high-quality videos that have been recognized within the community for their exceptional visual appeal. This set helps to enhance the aesthetic quality of the videos produced by the model. Specifically, from a large dataset of filtered videos, we select 50k videos of exceptionally high quality. The selection process involves multiple filters such as text and optical character recognition, aesthetic scoring, video-text alignment, as well as positional and object detection. Additionally, human visual judgment plays a crucial role in the final selection to ensure the highest standards of visual quality are met.
This methodical approach to refining the model's output through the use of high-quality visual data ensures that the generated videos are not only accurate in terms of content but also aesthetically pleasing. This refinement helps stabilize video quality and aligns it more closely with human visual preferences, thereby enhancing the overall effectiveness and applicability of the generative model in real-world scenarios.


